RoboPIN: Grounded Embodied Reasoning via Pinned Chain-of-Thought

Embodied reasoning requires models to perceive task-relevant objects and spaces in physical environments and maintain consistent visual grounding throughout multi-step reasoning. However, current vision-language models rely on text-only or coordinate-augmented chain-of-thought, where entity references remain implicit and ambiguous. This may cause the reasoning process to decouple from visual evidence, entity references to drift across steps, and a causal disconnection between the reasoning trajectory and the final answer, with these problems further amplified in multi-view scenarios due to cross-view appearance changes. To address these issues, we propose Pinned Chain-of-Thought (PinCoT), a structured reasoning paradigm that pins every reasoning step to visual evidence. PinCoT introduces the concept of reasoning anchor, which binds each task-relevant entity to a structured visual anchor with entity name, unique identity, view index, and spatial grounding, enabling consistent entity tracking across reasoning steps and views. We build a fully automated data generation pipeline to construct PIN-170K, a high-quality PinCoT-formatted reasoning dataset. We then train RoboPIN through three-stage post-training that progressively injects embodied knowledge, structured reasoning ability, and process-supervised alignment, with rewards that directly constrain both anchor localization and identity consistency during reasoning. On 14 benchmarks covering embodied spatial reasoning, multi-view reasoning, and pointing, RoboPIN with only 4B parameters surpasses 7B level open-source embodied models on average, achieving a 12% average improvement over the strongest 7B baseline, Mimo-Embodied. Further analysis shows that PinCoT improves grounding accuracy and cross-step identity consistency, validating the effectiveness of process supervision.

==> ER_RoboPIN__Grounded_Embodied_Reasoning_via_Pinned_Chain_of_Thought/Makefile <==
TEX = main

.PHONY: all clean

all: $(TEX).pdf

$(TEX).pdf: $(TEX).tex sample-base.bib sections/*.tex iffyuan.cls
	pdflatex -interaction=nonstopmode $(TEX).tex
	bibtex $(TEX)
	pdflatex -interaction=nonstopmode $(TEX).tex
	pdflatex -interaction=nonstopmode $(TEX).tex

clean:
	$(RM) $(TEX).aux $(TEX).bbl $(TEX).blg $(TEX).log $(TEX).out \
	      $(TEX).toc $(TEX).lof $(TEX).lot $(TEX).fls $(TEX).fdb_latexmk \
	      $(TEX).synctex.gz


==> ER_RoboPIN__Grounded_Embodied_Reasoning_via_Pinned_Chain_of_Thought/sections/ablations.tex <==
\section{Ablation Study and Analysis}

In this section, we conduct ablation experiments in both embodied reasoning and multi-view reasoning settings to examine whether the performance gains of our model mainly arise from the proposed structured VIA-CoT design and the subsequent RFT optimization. To this end, we construct several model variants with different reasoning supervision formats and training strategies, and evaluate them on the corresponding benchmarks in each scenario. By comparing the resulting performance changes, we analyze the contribution of VIA-CoT and RFT to the final model performance.

\noindent\textbf{Experimental Setup.}
We compare eight configurations built around the Qwen3-VL-4B model family. The original Qwen3-VL-4B-Instruct serves as the base model for all supervised training variants and also provides the primary training baseline without any additional adaptation. We further include the off-the-shelf Qwen3-VL-4B-Thinking model as a reference baseline to compare against a native reasoning model.

Starting from each sampled ablation subset, we construct three supervision formats from the same underlying image--question--answer instances. The first is a \textbf{Direct} dataset that contains only the final answers and is used to train a standard QA model without intermediate reasoning. The second is a \textbf{CoT} dataset, where chain-of-thought traces are generated by Qwen3-VL-32B-Instruct. The third is a \textbf{VIA-CoT} dataset produced by our current pipeline, which provides structured reasoning traces with explicit visual anchors and identity tracking. For each supervision format, we evaluate both an SFT-only variant and a corresponding RFT-enhanced variant when applicable, yielding six trained variants in total. Across all ablation settings, except for differences in supervision format and the optional RFT stage, the remaining training-related settings are kept identical to ensure a controlled comparison.



\subsection{Embodied Reasoning Ablations}

We conduct the embodied reasoning ablation study on \textbf{EmbSpatial}, which is accompanied by corresponding data targeting embodied spatial reasoning capabilities.
For comparison, we extract a fixed evaluation subset consisting of 25K samples from EmbSpatial.

\begin{table}[htbp]
  \centering
  \small
  \setlength{\tabcolsep}{6pt}
  \caption{Embodied ablations on EmbSpatial.}
  \label{tab:embodied_ablation_main}
  \begin{tabular}{lc}
    \toprule
    Model & Accuracy $\uparrow$ \\
    \midrule
    Qwen3-VL-4B-Instruct & 77.1 \\
    Qwen3-VL-4B-Thinking & 78.9 \\
    \midrule
    Direct & 76.00 \\
    \hspace{0.8em}w/o RFT & 75.1 \\
    CoT & 79.23 \\
    \hspace{0.8em}w/o RFT & 79.1 \\
    \rowcolor{blue!10} VIA-CoT & \textbf{84.7} \\
    \hspace{0.8em}w/o RFT & 80.3 \\
    \bottomrule
  \end{tabular}
\end{table}


\subsection{Multi-view Reasoning Ablations}

We further evaluate the impact of structured reasoning in the multi-view setting on the \textbf{SAT} benchmark, where we focus on the \textbf{ego\_movement} and \textbf{obj\_movement} subtasks.
For comparison, we construct fixed evaluation subsets from these two SAT subtasks and evaluate all supervision variants under the same protocol.

\begin{table}[htbp]
  \centering
  \small
  \setlength{\tabcolsep}{6pt}
  \caption{Multi-view ablations on the SAT \textit{ego\_movement} and \textit{obj\_movement} subtasks.}
  \label{tab:multiview_ablation}
  \begin{tabular}{lcc}
    \toprule
    Model & \shortstack{ego\_movement\\Accuracy $\uparrow$} & \shortstack{obj\_movement\\Accuracy $\uparrow$} \\
    \midrule
    Qwen3-VL-4B-Instruct & 79.3 & 39.1 \\
    Qwen3-VL-4B-Thinking & 82.6 & 60.9 \\
    \midrule
    Direct & 73.9 & 60.8 \\
    \hspace{0.8em}w/o RFT & 39.1 & 39.1 \\
    CoT & \textbf{100} & 82.6 \\
    \hspace{0.8em}w/o RFT & 91.3 & 73.9 \\
    \rowcolor{blue!10} VIA-CoT & \textbf{100} & \textbf{87.0} \\
    \hspace{0.8em}w/o RFT & 87.0 & 78.3 \\
    \bottomrule
  \end{tabular}
\end{table}


\subsection{Reward Function Ablations}

To further isolate the contribution of individual reward terms introduced in Section~\ref{sec:training}, we conduct a reward-function ablation study in the same embodied setting as above. Concretely, we reuse the same EmbSpatial training data and the same fixed 25K-sample EmbSpatial evaluation subset used in the embodied reasoning ablations. All training and evaluation settings are kept identical to the full VIA-CoT + RFT model, except that we remove one reward term at a time during Stage 3 RFT.

In particular, we examine two reward components that are directly related to the proposed grounded reasoning behavior: the spatial reward $R_{\text{spatial}}$, which supervises intermediate visual grounding, and the ID-tracking reward $R_{\text{consistency}}$, which encourages consistent entity references throughout the reasoning trajectory. The format reward and accuracy reward are kept unchanged in these ablations.

\begin{table}[htbp]
  \centering
  \small
  \setlength{\tabcolsep}{6pt}
  \caption{Reward-function ablations on EmbSpatial.}
  \label{tab:reward_ablation_embodied}
  \begin{tabular}{lc}
    \toprule
    Model & Accuracy $\uparrow$ \\
    \midrule
     VIA-CoT & \textit{80.3} \\
    \rowcolor{blue!10} VIA-CoT + RFT & \textit{84.7} \\
    \hspace{0.8em}w/o Spatial Reward & 81.2 \\
    \bottomrule
  \end{tabular}
\end{table}

This ablation is designed to distinguish whether the gains from RFT mainly come from better intermediate spatial grounding or from more stable ID tracking. After the results are filled in, the relative performance drop of each variant can be used to quantify the importance of the corresponding reward component under the embodied evaluation setting.



\subsection{Analysis.}
The results reveal a clear trend as the reasoning format becomes more structured. 
Direct supervision provides limited support for multi-step reasoning in multi-view settings. 
Introducing chain-of-thought reasoning improves performance by exposing intermediate reasoning steps. 
Structured VIA-CoT further enhances performance by explicitly grounding reasoning steps to visual anchors and maintaining consistent object identities across views. 
Finally, reinforcement fine-tuning provides additional gains by aligning reasoning trajectories with task-level objectives.

==> ER_RoboPIN__Grounded_Embodied_Reasoning_via_Pinned_Chain_of_Thought/sections/abstract.tex <==
\abstract{%
Embodied reasoning requires models to perceive task-relevant objects and spaces in physical environments and maintain consistent visual grounding throughout multi-step reasoning. However, current vision-language models rely on text-only or coordinate-augmented chain-of-thought, where entity references remain implicit and ambiguous. This may cause the reasoning process to decouple from visual evidence, entity references to drift across steps, and a causal disconnection between the reasoning trajectory and the final answer, with these problems further amplified in multi-view scenarios due to cross-view appearance changes. To address these issues, we propose Pinned Chain-of-Thought (\pincot{}), a structured reasoning paradigm that pins every reasoning step to visual evidence. \pincot{} introduces the concept of \reasoninganchor{}, which binds each task-relevant entity to a structured visual anchor with entity name, unique identity, view index, and spatial grounding, enabling consistent entity tracking across reasoning steps and views. We build a fully automated data generation pipeline to construct \dataset{}, a high-quality \pincot{}-formatted reasoning dataset. We then train \method{} through three-stage post-training that progressively injects embodied knowledge, structured reasoning ability, and process-supervised alignment, with rewards that directly constrain both anchor localization and identity consistency during reasoning. On 14 benchmarks covering embodied spatial reasoning, multi-view reasoning, and pointing, \method{} with only 4B parameters surpasses 7B level open-source embodied models on average, achieving a 12\% average improvement over the strongest 7B baseline, Mimo-Embodied. Further analysis shows that \pincot{} improves grounding accuracy and cross-step identity consistency, validating the effectiveness of process supervision.
}


==> ER_RoboPIN__Grounded_Embodied_Reasoning_via_Pinned_Chain_of_Thought/sections/con_ack.tex <==

\section{Conclusion}

We present Pinned Chain-of-Thought (PinCoT), a structured reasoning paradigm that pins every reasoning step onto visual evidence by unifying semantic name and spatial localization into a structured reasoning variable, enabling persistent entity tracking across reasoning steps and viewpoints. We build a fully automated data generation pipeline to construct the PIN-170K reasoning dataset. Then we train RoboPIN through three-stage progressive post-training, where the RFT stage employs a composite reward function that simultaneously supervises the reasoning process and the final answer, effectively ensuring the localization accuracy of reasoning anchors. Across 14 embodied VLM benchmarks, RoboPIN with only 4B parameters achieves an average improvement of 12\% over the strongest 7B baseline Mimo-Embodied. Overall, our work demonstrates that explicitly anchoring
  the reasoning process to visual evidence is an effective and scalable path toward enhancing the spatial reasoning capabilities of embodied VLMs. Various analytical experiments further confirm that PinCoT substantially improves the localization accuracy and cross-step identity consistency.
  Although RoboPIN already surpasses larger-scale embodied VLMs, the current work validates PinCoT only at the 4B parameter scale. In the future, scaling up data and model size is expected to further improve performance, and we plan to extend PinCoT to 3D spatial localization and long-horizon
  planning, exploring the potential of reasoning anchors in more complex physical interactions.


==> ER_RoboPIN__Grounded_Embodied_Reasoning_via_Pinned_Chain_of_Thought/sections/experiment.tex <==
\section{Experiments}

We evaluate \method{} on embodied spatial reasoning (Sec.~\ref{sec:embodied_reasoning}), point-level grounding (Sec.~\ref{sec:pointing}), and real-world robot execution (Sec.~\ref{sec:real_world}). We then ablate the contributions of \pincot{} and the three-stage training recipe (Sec.~\ref{sec:ablation}), and analyze how process supervision improves reasoning quality and consistency (Sec.~\ref{sec:reasoning_analysis}). Finally, we verify that our embodied alignment preserves general vision-language capabilities without catastrophic forgetting, with detailed results provided in Appendix D.

\subsection{Embodied Cognition and Spatial Reasoning}
\label{sec:embodied_reasoning}
\textbf{Setup.} We evaluate the embodied cognition and spatial reasoning capabilities of our model across 9 benchmarks encompassing 13 distinct capability dimensions. These include ERQA~\cite{team2025gemini}, CV-Bench~\cite{tong2024cambrian}, EmbSpatial~\cite{du2024embspatial}, SAT~\cite{ray2024sat}, RoboSpatial~\cite{song2025robospatial}, Robo-VQA~\cite{sermanet2024robovqa}, CrossPoint~\cite{wang2025towards}, MVRoboBench~\cite{feng2025seeing}, and BLINK~\cite{fu2024blink}. These benchmarks comprehensively cover various aspects of spatial understanding, object localization, and physical reasoning. To rigorously assess performance, we compare \method{} against two leading closed-source models: GPT-5~\cite{singh2025openai} and Gemini-2.5-Pro~\cite{comanici2025gemini}, alongside seven competitive open-source vision-language models equipped with advanced spatial reasoning and grounding capabilities. These include generalist multi-modal models (Qwen3-VL~\cite{bai2025qwen3} and InternVL3.5~\cite{wang2025internvl3}), as well as recent domain-specific models designed for embodied reasoning (RoboBrain2.0~\cite{team2025robobrain}, VeBrain~\cite{luo2025visual}, Mimo-Embodied~\cite{hao2025mimo}, Pelican-VL~\cite{zhang2025pelican}, and Embodied-R1~\cite{yuan2025embodied}).

\textbf{Results.} As detailed in Table~\ref{tab:main_reasoning_results}, \method{} demonstrates exceptional general spatial reasoning capabilities. It achieves the best open-source results on EmbSpatial, SAT, and RoboSpatial, highlighting the strong advantage of \pincot{} in tasks that require comparing relative object positions and tracking spatial changes. Across the other embodied cognition benchmarks, our model consistently performs within the first tier. Furthermore, on multi-view specific evaluations, \method{} ranks first on CrossPoint, as well as the Multi-View and Visual Correspondence subsets of BLINK. This indicates that the universal identity design across views effectively facilitates stable object correspondence, enhancing the model's multi-view reasoning proficiency.


\begin{table*}[t]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{2.8pt}
  \caption{Performance on spatial reasoning benchmarks. \textbf{Bold} and \underline{underlined} denote the best and second open-source results.}
  \label{tab:main_reasoning_results}
  \resizebox{\textwidth}{!}{%
  \begin{tabular}{lcccccccc|cc|cccc}
  \toprule
  \multirow{2}{*}{Model} & \multirow{2}{*}{Params} & \multirow{2}{*}{ERQA} & \multirow{2}{*}{\shortstack{CV-Bench}} & \multirow{2}{*}{\shortstack{EmbSpatial}} & \multirow{2}{*}{SAT} & \multirow{2}{*}{\shortstack{RoboSpatial}} & \multirow{2}{*}{\shortstack{RoboVQA}} &
  \multirow{2}{*}{CrossPoint} & \multicolumn{2}{c|}{\textbf{MV-RoboBench}} & \multicolumn{4}{c}{\textbf{BLINK}} \\
  & & & & & & & & & CrossV. Match & Traj. Sel & Multi. View & \shortstack{Vis. Corr.} & \shortstack{Spat. Rel.} & \shortstack{Rel. Depth} \\
  \midrule
  \rowcolor{gray!10} \multicolumn{15}{l}{\textit{Closed-source models}} \\
  GPT-5 & - & 54.5 & 84.5 & 78.3 & 83.3 & 54.1 & 33.1 & 33.0 & 29.0 & 54.5 & 45.8 & 77.3 & 90.2 & 82.3 \\
  Gemini-2.5-Pro & - & 55.7 & 84.6 & 78.7 & 76.7 & 59.9 & 33.9 & 37.1 & 39.5 & 65.5 & 46.6 & 78.5 & 85.3 & 86.3 \\
  \rowcolor{gray!10} \multicolumn{15}{l}{\textit{Open-source generalist models}} \\
  Qwen3-VL & 4B & 41.8 & 85.0 & \underline{77.1} & 70.7 & 59.4 & 41.1 & 29.3 & \underline{24.0} & 31.0 & \underline{51.1} & \underline{88.4} & \underline{84.6} & 85.5 \\
  InternVL3.5 & 8B & 41.0 & 81.5 & 70.3 & 55.3 & 51.1 & 28.6 & 19.2 & 21.5 & \underline{35.0} & 47.4 & 72.7 & 81.8 & 78.2 \\
  \rowcolor{gray!10} \multicolumn{15}{l}{\textit{Open-source embodied models}} \\
  RoboBrain2.0 & 7B & 38.5 & \underline{85.8} & 76.3 & 75.3 & 54.2 & 57.5 & 26.0 & 21.0 & 26.0 & 48.1 & 46.5 & 80.4 & 80.7 \\
  VeBrain & 7B & 37.3 & 79.7 & 70.5 & 58.0 & 42.5 & 42.4 & 20.2 & 18.0 & 30.0 & 46.6 & 48.8 & 83.2 & 67.7 \\
  Mimo-Embodied & 7B & \textbf{46.8} & \textbf{88.8} & 76.2 & 54.6 & \underline{61.8} & \textbf{62.0} & \underline{36.8} & 21.1 & 34.0 & 26.3 & 83.2 & 77.6 & \textbf{94.4} \\
  Pelican-VL & 7B & 39.8 & 78.9 & 73.2 & 54.6 & 57.5 & \underline{58.5} & 23.8 & 23.0 & 32.5 & 47.3 & 63.3 & \underline{84.6} & 75.0 \\
  Embodied-R1 & 3B & 35.2 & 82.7 & 67.4 & \underline{76.3} & 47.4 & 51.8 & 25.2 & 21.5 & 26.5 & 40.6 & 50.0 & 76.9 & 79.8 \\
  \midrule
  \rowcolor{blue!10} \method{} & 4B & \underline{44.0} & 85.5 & \textbf{83.1} & \textbf{78.0} & \textbf{66.6} & 56.1 & \textbf{72.2} & \textbf{26.0} & \textbf{35.5} & \textbf{72.9} & \textbf{89.5} & \textbf{87.4} & \underline{87.1} \\
  \bottomrule
  \end{tabular}%
  }
\end{table*}

\subsection{Embodied Pointing and Location}
\label{sec:pointing}
\textbf{Setup.} We next examine point-level grounding ability by evaluating on five distinct benchmarks: VABench-P~\cite{yuan2025seeing}, Where2Place~\cite{yuan2024robopoint}, RefSpatial~\cite{zhou2025roborefer}, RoboRefit~\cite{lu2023vl}, and RoboAfford~\cite{tang2025roboafford}. 
% \textbf{Results.} As shown in Table~\ref{tab:main_pointing_results}, \method{} achieves the best open-source performance on RefSpatial, RoboRefit, and RoboAfford, while remaining competitive on VABench-P and Where2Place. The strongest gains appear on tasks that require the model to align a linguistic instruction with a functionally meaningful point or region, suggesting that the structured reasoning trace improves not only final-answer selection but also the precision of point-level grounding.

\textbf{Results.} As shown in Table~\ref{tab:main_pointing_results}, \method{} achieves the best open-source performance on RefSpatial, RoboRefit, and RoboAfford. We note that Embodied-R1, as a model specifically designed and trained for pointing tasks, shows strong performance on VABench-P and Where2Place. Despite being a general-purpose embodied reasoning model, \method{} remains competitive on two benchmarks while significantly outperforming Embodied-R1 on broader spatial reasoning tasks, demonstrating a more balanced capability profile. 

\begin{table}[t]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{6pt}
  \caption{Performance on pointing benchmarks. \textbf{Bold} and \underline{underlined} values denote the best and second-best open-source results.}
  \label{tab:main_pointing_results}
  \begin{adjustbox}{max width=\columnwidth}
  \begin{tabular}{lcccccc}
    \toprule
    Model & Params & \shortstack{VABench-P} & \shortstack{Where2Place} & \shortstack{Ref-Spatial} & \shortstack{Robo-Refit} & \shortstack{Robo-Afford} \\
    \midrule
    \rowcolor{gray!10} \multicolumn{7}{l}{\textit{Closed-source models}} \\
    GPT-5 & - & 31.1 & 39.7 & 21.6 & 44.7 & 30.0 \\
    Gemini-2.5-Pro & - & 21.7 & 49.6 & 36.5 & 38.4 & 23.4 \\
    \rowcolor{gray!10} \multicolumn{7}{l}{\textit{Open-source generalist models}} \\
    Qwen3-VL & 4B & 30.6 & \underline{67.7} & 43.0 & \underline{86.1} & \underline{70.1} \\
    InternVL3.5 & 8B & 23.0 & 34.8 & 16.8 & 30.8 & 31.5 \\
    \rowcolor{gray!10} \multicolumn{7}{l}{\textit{Open-source embodied models}} \\
    RoboBrain2.0 & 7B & 41.0 & 63.6 & 32.5 & 70.4 & 51.5 \\
    VeBrain & 7B & 1.7 & 12.3 & 0.3 & 32.2 & 2.1 \\
    Mimo-Embodied & 7B & 46.9 & 63.6 & \underline{48.0} & 82.3 & 69.8 \\
    Pelican-VL & 7B & 14.5 & 57.8 & 37.5 & 74.9 & 63.4 \\
    Embodied-R1 & 3B & \textbf{66.0} & \textbf{69.5} & 39.7 & 85.6 & 67.2 \\
    \midrule
    \rowcolor{blue!10} \method{} & 4B & \underline{65.0} & 62.0 & \textbf{50.5} & \textbf{89.0} & \textbf{72.8} \\
    \bottomrule
  \end{tabular}%
  \end{adjustbox}
\end{table}



\begin{table*}[t]
  \begin{minipage}[t]{0.49\textwidth}
    \vspace{0pt}
    \centering
    \scriptsize
    \setlength{\tabcolsep}{5pt}
    \captionof{table}{Reasoning process analysis on EmbSpatial.
     A-Cov: Anchor Coverage; AC: Anchor Correctness; CS-IDCov: Cross-Step identity Coverage.}
    \label{tab:reasoning_process_combined}
    \begin{adjustbox}{max width=\linewidth,center}
      \begin{tabular}{lccc}
        \toprule
        Model & A-Cov (\%) & AC (\%) & CS-IDCov (\%) \\
        \midrule
        \method{} &  \textbf{100.0} & \textbf{89.1} & \textbf{99.9} \\
        \hspace{0.8em}w/o RFT  & 96.3 & 87.0 & 18.8 \\
        \bottomrule
      \end{tabular}
    \end{adjustbox}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.48\textwidth}
    \vspace{0pt}
    \centering
    \scriptsize
    \captionof{table}{Error propagation on EmbSpatial.}
    \label{tab:anchor_answer_risk}
    \begin{adjustbox}{max width=\linewidth,center}
      \begin{tabular}{lccc}
        \toprule
        & \multicolumn{2}{c}{Answer Error Rate (\%)} & \\
        \cmidrule(lr){2-3}
        Model & w/ Faulty Anchor & w/ Correct Anchor & Risk Ratio \\
        \midrule
        \method{} & 29.2 & 13.2 & 2.2 \\
        \bottomrule
      \end{tabular}
    \end{adjustbox}
  \end{minipage}
\end{table*}

\begin{table}[t]
\caption{Cross-view reasoning consistency on CrossPoint. Acc: Overall Accuracy; ID-Trans: Shared-ID Transfer Rate; Trans-Acc: Accuracy given successful ID transfer.}
\label{tab:crosspoint_consistency}
\centering
\small
\setlength{\tabcolsep}{8pt}
\begin{tabular}{lccc}
  \toprule
  Model & Acc (\%) & ID-Trans (\%) & Trans-Acc (\%) \\
  \midrule
   \method{} & \textbf{71.1} & \textbf{86.3} & \textbf{72.1} \\
  \hspace{0.8em}w/o RFT & 62.5 & 60.6 & 61.1 \\
  \bottomrule
\end{tabular}
\end{table}


\subsection{Real-World Robot Evaluation}
\label{sec:real_world}
We conduct zero-shot real-world evaluations using an xArm robot. The system is equipped with two RGB cameras: a static camera observing the tabletop scene and a wrist-mounted camera. Given a language instruction, the model predicts target points via visual grounding, which are then executed using the point-based motion planning pipeline from Embodied-R1~\cite{yuan2025embodied}.

\textbf{Tasks.} We design three types of complex manipulation tasks to evaluate spatial reasoning, multi-view understanding, and long-horizon planning:

\textbf{(1) Spatial reasoning task}: \textit{“Pick up the duck in front of two toys and place it to the middle plate among plates.”}

\textbf{(2) Multi-view reasoning task}: \textit{“Pick up the duck behind two toys and place it to the plate in front of the two toys.”}

\textbf{(3) Long-horizon task}: \textit{“Pick up yellow objects located outside the plates and place into the yellow plate.”}

To rigorously ensure robustness, we extensively randomize object instances, distractor placements, and overall scene layouts for each task. We conduct 20 distinct trials per setting under these varied conditions to compute the success rate.

\textbf{Results.} Table~\ref{tab:realworld_results} reports the success rates of different methods, including RoboBrain2-7B and Mimo-Embodied-7B. In multi-view tasks, baseline models tend to rely solely on the static camera and often select incorrect targets, failing to utilize the wrist-view information. In contrast, our model effectively integrates multi-view observations and demonstrating enhanced reliability in identifying the target object compared to the baselines.

In spatial reasoning tasks, our model also achieves consistently higher accuracy, reflecting a stronger capacity for interpreting spatial relations and resolving ambiguous object configurations. For the long-horizon task, RoboPIN predicts keypoints step-by-step and outperforms other models at each step, leading to a substantially higher overall success rate. Figure~\ref{fig:realworld_robot} illustrates representative execution sequences alongside the predicted anchor points for multi-view and spatial tasks, visually confirming the model's ability to ground its reasoning in precise spatial locations.

\begin{figure*}[t]
  \centering
  \includegraphics[width=\textwidth]{figures/real_image.png}
  \caption{Real-world robot visualization. Left: robot execution. Right: predicted anchor points during manipulation. R.B and M.E denote RoboBrain2.0 and Mimo-Embodied.}
  \label{fig:realworld_robot}

  \vspace{0.5em}

  \captionof{table}{Real-world robot evaluation. Each setting is evaluated over 20 independent trials.}
  \label{tab:realworld_results}
  \centering
  \small
  \begin{tabular}{lccc}
    \toprule
    \textbf{Task} 
    & \shortstack{RoboBrain2.0} & \shortstack{Mimo-Embodied} & \shortstack{\method{}} \\
    \midrule
      Spatial         & 12/20 & 7/20  & \textbf{20/20} \\
      Multi-view      & 1/20  & 0/20  & \textbf{14/20} \\
      Long-horizon    & 5/20  & 3/20  & \textbf{11/20} \\
    \bottomrule
  \end{tabular}
\end{figure*}




\subsection{Ablation Study}
\label{sec:ablation}

In this section, we conduct ablation studies on three key components: the reasoning format, the reward design, and the three-stage training pipeline.
For the format and reward ablations, we use identical training hyperparameters on fixed training subsets to isolate the effects of reasoning format and reward design.

\textbf{Performance Comparison of Reasoning Formats.} We compare four spatial representations: standard text-only CoT (\textit{Text CoT}), coordinate-augmented CoT (\textit{Coord CoT}), coordinate CoT with explicit IDs (\textit{Coord CoT w/ ID}), and our proposed \pincot{} which utilizes point-based anchors with IDs. As shown in Table~\ref{tab:format_rft_ablation}, introducing explicit reasoning generally improves upon the non-reasoning baseline, but the spatial representation plays a critical role. Across the two benchmarks, \pincot{} generally outperforms other formats, and its advantage is significantly amplified with the introduction of RFT. Notably, under standard SFT, \pincot{} underperforms \textit{Coord CoT} on EmbSpatial. However, once RFT is applied, \pincot{} successfully surpasses \textit{Coord CoT}. This reversal suggests that \pincot{} provides a more stable and effective reasoning interface, but requires RFT to fully realize its potential. Furthermore, comparing \pincot{} with \textit{Coord CoT w/ ID}, which shares the same ID tracking mechanism but uses box coordinates instead of points, \pincot{} consistently outperforms it under both SFT and RFT settings. This confirms that point-based anchors serve as a more effective spatial primitive for reasoning, likely due to their lightweight and action-oriented nature that aligns better with embodied tasks.

\begin{figure*}[!t]
  \centering
  \includegraphics[width=\textwidth]{figures/sample_v4.pdf}
  \caption{Qualitative analysis of grounded reasoning.}
  \label{fig:qualitative_reasoning}
\end{figure*}


% \begin{table}[t]
%   \caption{Ablation of reasoning format and RFT. The first row indicates the Qwen3-VL-4B-Instruct baseline. All compared variants use the same training recipe and data subsets.}
%   \label{tab:format_rft_ablation}
%   \centering
%   \small
%   \setlength{\tabcolsep}{4pt}
%   \begin{tabular}{lcc|cc}
%     \toprule
%     \multicolumn{3}{c|}{\textbf{Reasoning Design}} & \multicolumn{2}{c}{\textbf{Performance}} \\
%     \cmidrule(lr){1-3} \cmidrule(lr){4-5}
%     Format & SFT & RFT & EmbSpatial & SAT \\
%     \midrule
%     Baseline & $\times$ & $\times$ & 77.1 & 70.7 \\
%     Text CoT & $\checkmark$ & $\times$ & 78.9 & 74.0 \\
%     Text CoT & $\checkmark$ & $\checkmark$ & 79.3 & 76.3 \\
%     Coord CoT & $\checkmark$ & $\times$ & 81.7 & 67.3 \\
%     Coord CoT & $\checkmark$ & $\checkmark$ & 83.1 & 74.0 \\
%     Coord CoT w/ ID & $\checkmark$ & $\times$ & 78.6 & 70.7 \\
%     Coord CoT w/ ID & $\checkmark$ & $\checkmark$ & 81.5 & 76.0 \\
%     \pincot{} & $\checkmark$ & $\times$ & 80.3 & 74.0 \\
%     \pincot{} & $\checkmark$ & $\checkmark$ & \textbf{84.7} & \textbf{78.7} \\
%     \bottomrule
%   \end{tabular}
% \end{table}


\textbf{Ablation of Reward Components.}
We further ablate the two core reward components in RFT: the Pin reward for anchor localization and the Consistency reward for entity references. As shown in Table~\ref{tab:reward_ablation}, removing either component leads to a clear performance drop, confirming that both spatially accurate anchors and identity-consistent reasoning are necessary for strong embodied reasoning performance. Notably, removing the Pin reward causes a larger degradation ($-$2.7) than removing the Consistency reward ($-$2.0), suggesting that anchor localization quality is the more fundamental bottleneck for embodied reasoning.

% \begin{table}[t]
%   \caption{Ablation of reward components on EmbSpatial.}
%   \label{tab:reward_ablation}
%   \centering
%   \begin{tabular}{lc}
%     \toprule
%     Setting & EmbSpatial \\
%     \midrule
%     \method{} & \textbf{84.7} \\
%     \hspace{0.8em}w/o Pin reward & 82.0 \\
%     \hspace{0.8em}w/o Consistency reward & 82.7 \\
%     \bottomrule
%   \end{tabular}
% \end{table}


\textbf{Performance Comparison of the Three-Stage Training.}
We further analyze how model performance progresses across different training stages based on average scores over embodied reasoning and pointing tasks. As shown in Table~\ref{tab:three_stage_ablation}, embodied reasoning improves progressively as additional stages are introduced: CoT-SFT yields a +5.0 gain over SFT alone, and RFT provides a further +5.7 improvement. This suggests that our three-stage recipe primarily strengthens high-level embodied spatial reasoning, while effectively preserving the fundamental point-level localization capabilities.

% \begin{table}[t]
%   \caption{Ablation of the three-stage training recipe.}
%   \label{tab:three_stage_ablation}
%   \centering
%   \begin{tabular}{ccc|cc}
%     \toprule
%     \multicolumn{3}{c|}{\textbf{Training Stages}} & \multicolumn{2}{c}{\textbf{Avg-Performance}} \\
%     \cmidrule(lr){1-3} \cmidrule(lr){4-5}
%     SFT & CoT-SFT & RFT & Spatial & Point \\
%     \midrule
%     $\checkmark$ & $\times$ & $\times$ & 57.0 & 66.0 \\
%     $\checkmark$ & $\checkmark$ & $\times$ & 62.0 & 63.6 \\
%     $\checkmark$ & $\checkmark$ & $\checkmark$ & \textbf{67.7} & \textbf{67.9} \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\begin{table*}[t]
  \centering
  \scriptsize
  \setlength{\tabcolsep}{4pt}
  \caption{Ablation of reasoning format and RFT. The first row indicates the Qwen3-VL-4B-Instruct baseline. All compared variants use the same training recipe and data subsets.}
  \label{tab:format_rft_ablation}
  \begin{adjustbox}{max width=\textwidth,center}
    \begin{tabular}{lcc|cc}
      \toprule
      \multicolumn{3}{c|}{\textbf{Reasoning Design}} & \multicolumn{2}{c}{\textbf{Performance}} \\
      \cmidrule(lr){1-3} \cmidrule(lr){4-5}
      Format & SFT & RFT & EmbSpatial & SAT \\
      \midrule
      Baseline & $\times$ & $\times$ & 77.1 & 70.7 \\
      Text CoT & $\checkmark$ & $\times$ & 78.9 & 74.0 \\
      Text CoT & $\checkmark$ & $\checkmark$ & 79.3 & 76.3 \\
      Coord CoT & $\checkmark$ & $\times$ & 81.7 & 67.3 \\
      Coord CoT & $\checkmark$ & $\checkmark$ & 83.1 & 74.0 \\
      Coord CoT w/ ID & $\checkmark$ & $\times$ & 78.6 & 70.7 \\
      Coord CoT w/ ID & $\checkmark$ & $\checkmark$ & 81.5 & 76.0 \\
      \pincot{} & $\checkmark$ & $\times$ & 80.3 & 74.0 \\
      \pincot{} & $\checkmark$ & $\checkmark$ & \textbf{84.7} & \textbf{78.7} \\
      \bottomrule
    \end{tabular}
  \end{adjustbox}
\end{table*}

\begin{table*}[t]
  \begin{minipage}[t]{0.38\textwidth}
    \vspace{0pt}
    \centering
    \scriptsize
    \captionof{table}{Ablation of reward components on EmbSpatial.}
    \label{tab:reward_ablation}
    \begin{adjustbox}{max width=\linewidth,center}
      \begin{tabular}{lc}
        \toprule
        Setting & EmbSpatial \\
        \midrule
        \method{} & \textbf{84.7} \\
        \hspace{0.8em}w/o Pin reward & 82.0 \\
        \hspace{0.8em}w/o Consistency reward & 82.7 \\
        \bottomrule
      \end{tabular}
    \end{adjustbox}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.59\textwidth}
    \vspace{0pt}
    \centering
    \scriptsize
    \captionof{table}{Ablation of the three-stage training recipe.}
    \label{tab:three_stage_ablation}
    \begin{adjustbox}{max width=\linewidth,center}
      \begin{tabular}{ccc|cc}
        \toprule
        \multicolumn{3}{c|}{\textbf{Training Stages}} & \multicolumn{2}{c}{\textbf{Avg-Performance}} \\
        \cmidrule(lr){1-3} \cmidrule(lr){4-5}
        SFT & CoT-SFT & RFT & Spatial & Point \\
        \midrule
        $\checkmark$ & $\times$ & $\times$ & 57.0 & 66.0 \\
        $\checkmark$ & $\checkmark$ & $\times$ & 62.0 & 63.6 \\
        $\checkmark$ & $\checkmark$ & $\checkmark$ & \textbf{67.7} & \textbf{67.9} \\
        \bottomrule
      \end{tabular}
    \end{adjustbox}
  \end{minipage}
\end{table*}

\subsection{Reasoning Process Analysis}
\label{sec:reasoning_analysis}

To understand why \method{} achieves superior performance, we analyze the intermediate reasoning process on EmbSpatial (which provides ground-truth bounding boxes) and CrossPoint (for cross-view evaluation).

\textbf{Anchor Quality and Identity Consistency.} As shown in Table~\ref{tab:reasoning_process_combined}, \method{} achieves full anchor coverage (100.0\%) and high anchor correctness (89.1\%), both of which degrade without RFT. However, the key difference lies in identity tracking: without RFT, the model rarely sustains ID-based reasoning across steps (18.8\%) despite reasonably accurate anchors, whereas with RFT it achieves 99.9\% cross-step coverage. This shows that process supervision enforces a stable identity-aware reasoning mechanism beyond merely improving anchor quality. We further visualize the inference process on representative examples in Figure~\ref{fig:qualitative_reasoning}, confirming that such identity-aware tracking eliminates ambiguous textual references and ensures strong cross-step and cross-view consistency.




% \begin{table}[t]
%   \caption{Reasoning process analysis on EmbSpatial.
%    A-Cov: Anchor Coverage; AC: Anchor Correctness; CS-IDCov: Cross-Step identity Coverage.}
%   \label{tab:reasoning_process_combined}
%   \centering
%   \small
%   \setlength{\tabcolsep}{5pt}
%   \begin{tabular}{lccc}
%     \toprule
%     Model & A-Cov (\%) & AC (\%) & CS-IDCov (\%) \\
%     \midrule
%     \method{} &  \textbf{100.0} & \textbf{89.1} & \textbf{99.9} \\
%     \hspace{0.8em}w/o RFT  & 96.3 & 87.0 & 18.8 \\
%     \bottomrule
%   \end{tabular}
% \end{table}

\textbf{Error Propagation from Reasoning to Answer.} As shown in Table~\ref{tab:anchor_answer_risk}, samples with faulty anchors exhibit roughly $2.2\times$ higher answer-error rates than those with correct anchors, confirming that reliable spatial grounding is a critical prerequisite for robust reasoning.

% \begin{table}[t]
%   \caption{Error propagation on EmbSpatial.}
%   \label{tab:anchor_answer_risk}
%   \centering
%   \small
%   \begin{tabular}{lccc}
%     \toprule
%     & \multicolumn{2}{c}{Answer Error Rate (\%)} & \\
%     \cmidrule(lr){2-3}
%     Model & w/ Faulty Anchor & w/ Correct Anchor & Risk Ratio \\
%     \midrule
%     \method{} & 29.2 & 13.2 & 2.2 \\
%     \bottomrule
%   \end{tabular}
% \end{table}



\textbf{Cross-view Consistency.} We evaluate the Pointing and Judgement subsets of CrossPoint, measuring overall accuracy (\textit{Acc}), shared-ID transfer rate across views (\textit{ID-Trans}), and conditional accuracy given successful transfer (\textit{Trans-Acc}). As shown in Table~\ref{tab:crosspoint_consistency}, \method{} consistently maintains shared-identity transfer across views (86.3\%), and when this transfer succeeds, predictions become highly reliable (72.1\%). Removing RFT substantially weakens this behavior (ID-Trans drops to 60.6\%), accompanied by a clear performance decline. These findings confirm that process supervision is the critical driver enforcing explicit cross-view correspondence.



==> ER_RoboPIN__Grounded_Embodied_Reasoning_via_Pinned_Chain_of_Thought/sections/introduction.tex <==
\section{Introduction}
% [NEW] --- begin new introduction ---
Embodied reasoning is a core capability for intelligent systems operating in the physical world~\cite{sermanet2024robovqa,chen2026egoplan,team2025gemini}. Tasks such as spatial reasoning, fine-grained pointing, and long-horizon planning require models to accurately perceive task-relevant objects and spatial regions in complex environments, while maintaining tight coupling between reasoning steps and visual evidence throughout multi-step inference~\cite{chen2024spatialvlm,cheng2024spatialrgpt,yuan2024robopoint,cheng2025pointarena,song2025robospatial}.

Despite the necessity of this tight coupling, current Vision-Language Models (VLMs) struggle to maintain it during embodied tasks.~\cite{du2024embspatial,song2025robospatial,fu2024blink}. Although chain-of-thought reasoning has advanced beyond pure text into multimodal and visually grounded forms~\cite{zhang2023multimodal}, existing methods still fall short on reasoning consistency. Multimodal chain-of-thought methods~\cite{mitra2024compositional,zheng2023ddcot,shao2024visual} incorporate visual information into the reasoning process, but reasoning steps remain largely textual and lack explicit spatial grounding. Coordinate-augmented approaches~\cite{chen2023shikra,li2025vocot,liao2024reasoning} go further by embedding coordinates or bounding boxes into reasoning chains, yet these spatial references are often isolated and lack explicit identity tracking across steps. As illustrated in Figure~\ref{fig:teaser}, this leads to two core problems. First, \textbf{reasoning decouples from visual evidence}: entity references within the reasoning process are implicit textual descriptions that cannot guarantee each step looks at the correct target, and cross-step entity references are prone to drift, especially when multiple instances of the same category co-exist in the scene. Second, \textbf{reasoning-to-answer misalignment}: when intermediate steps suffer from reference drift, the final answer loses its reliable visual grounding. Consequently, a model might correctly analyze object~A initially, but silently shift its attention and point to object~B in the final prediction. Current paradigms fail to detect this disconnection because the underlying causal chain is broken. These issues are further amplified in multi-view settings, these problems are further amplified because the same object undergoes appearance changes across viewpoints~\cite{wang2025towards,feng2025seeing,yang2025mmsi}. We unify these issues as the \textit{reasoning consistency} problem in embodied reasoning, spanning cross-step and cross-view consistency. The root cause is the lack of a unified \textit{\reasoninganchor{}} mechanism to persistently bind visual evidence throughout reasoning.

To address these issues, we propose \textit{Pinned Chain-of-Thought} (\textit{\pincot{}}), a structured reasoning paradigm that ``pins'' every reasoning step onto visual evidence. The core of \pincot{} is the \textit{\reasoninganchor{}}: each task-relevant entity is bound to a structured visual anchor with a name, unique identity, view index, and spatial grounding, rather than a one-shot perceptual detection result. During reasoning, an entity is introduced with a full tag establishing its localization and identity upon first appearance; subsequent steps refer to the same entity via its ID, forming a verifiable chain. enables identity-consistent reasoning, which extends to multi-view settings where the same object shares its ID across different viewpoints. Unlike coordinate-embedding methods such as Shikra~\cite{chen2023shikra}, region-grounding approaches such as Ferret~\cite{you2023ferret}, and visual chain-of-thought methods such as VoCoT~\cite{li2025vocot}, \pincot{} does not perform static grounding external to the reasoning process, but rather treats these visual references as persistently trackable anchors within the reasoning chain. To obtain supervision in the \pincot{} format~\cite{shao2024visual,zawalski2024robotic}, we build a fully automated pipeline and use it to construct the \dataset{} reasoning dataset, as shown in Figure~\ref{fig:intro_overview}. The pipeline transforms multimodal data into \pincot{}-format reasoning supervision through three stages: semantic parsing, precise point grounding, and reasoning chain generation, incorporating dedicated quality assurance throughout the process.

Building on this framework and data, we train \method{} through SFT, CoT-SFT, and RFT three-stage post-training, which respectively inject embodied knowledge, structured reasoning ability, and process-supervised alignment~\cite{yuan2025embodied}. The RFT stage employs a composite reward function that simultaneously supervises the reasoning process and the final answer~\cite{lightman2023let}, effectively mitigating reference drift across reasoning steps.

Extensive experiments show that \method{} achieves best average performance across 14 benchmarks covering embodied spatial reasoning, multi-view reasoning, and pointing tasks~\cite{du2024embspatial,song2025robospatial,ray2024sat,wang2025towards,feng2025seeing,fu2024blink}. Further analysis confirms that \pincot{} substantially improves the localization accuracy of reasoning anchors and cross-step identity consistency, validating the effectiveness of process supervision on reasoning quality.
The main contributions are as follows:

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/teaser_v1.pdf}
    \caption{Comparison of three chain-of-thought paradigms for embodied reasoning. Text CoT relies on implicit textual descriptions with ambiguous entity references. Coord CoT embeds coordinates but lacks identity tracking, causing disconnection between reasoning and the final answer. \pincot{} (ours) pins each reasoning step to visual evidence via pinned reasoning anchors, ensuring identity-level traceability from the reasoning process to the final answer.}
    \label{fig:teaser}
\end{figure*}



\begin{itemize}[leftmargin=*,nosep]

\item We propose \textbf{\pincot{}}, introducing the \reasoninganchor{} concept that converts implicit visual attention during reasoning into explicit, trackable structured visual anchors, achieving cross-step and cross-view reasoning consistency.

\item We build a fully automated, high-quality data generation pipeline and construct the \dataset{} dataset, enabling large-scale generation of \pincot{}-format reasoning supervision.

\item We train \textbf{\method{}} with three-stage post-training and process-supervised rewards that jointly optimize reasoning process quality and answer correctness. Impressively, with only 4B parameters, \method{} achieves best average performance across 14 benchmarks spanning embodied spatial reasoning, pointing, and multi-view reasoning, outperforming 7B level open-source embodied models with a 12\% average improvement over the strongest 7B baseline Mimo-Embodied~\cite{hao2025mimo}.

\end{itemize}

==> ER_RoboPIN__Grounded_Embodied_Reasoning_via_Pinned_Chain_of_Thought/sections/keword.tex <==
\metadata[Keywords]{Embodied Reasoning, Spatial Reasoning, Multi-view Reasoning}
\metadata[\raisebox{-1.5pt}{\includegraphics[height=1.03em]{figures/github-logo.pdf}}\ Code]{\href{\codeurl}{\codeurl}}
\metadata[\raisebox{-1.5pt}{\includegraphics[height=0.96em]{figures/hf-logo.pdf}}\ Dataset]{\href{\dataseturl}{\dataseturl}}
\metadata[\faEnvelope\ Contact]{\href{mailto:quark404@tju.edu.cn}{quark404@tju.edu.cn}}


==> ER_RoboPIN__Grounded_Embodied_Reasoning_via_Pinned_Chain_of_Thought/sections/method.tex <==
% [NEW]
\section{Method}
\label{sec:method}

This section presents the complete framework of \method{}. Section~\ref{sec:pincot} defines the \pincot{} structured reasoning representation, including the design of \reasoninganchor{}s, the identity tracking mechanism, and its natural extension to multi-view settings. Section~\ref{sec:data} describes a fully automated data construction pipeline for generating high-quality \pincot{}-format reasoning supervision at scale. Section~\ref{sec:training} introduces the three-stage progressive training strategy and the process-supervised reward design.

\subsection{Pinned Chain-of-Thought Representation}
\label{sec:pincot}

As discussed in the introduction, although existing paradigms have introduced visual coordinates into language models, these spatial references are typically isolated and lack explicit identity tracking. This often causes the reasoning trajectory to decouple from visual evidence, leading to reference drift and inconsistency across steps. To address the reasoning consistency problem in embodied reasoning, we propose Pinned Chain-of-Thought (\pincot{}), whose core concept is the \textit{\reasoninganchor{}}.

A \reasoninganchor{} is fundamentally different from conventional visual grounding. Traditional grounding operations such as object detection and referring expression comprehension, operate primarily at the perceptual level and are not explicitly maintained throughout multi-step reasoning. Once an object is localized, the grounding result is typically not reused as a persistent variable. In contrast, a \reasoninganchor{} functions as a reasoning-level variable that unifies identity and grounding. Upon introduction, it binds an entity to a unique identity along with its spatial location and view context, and persists as a variable throughout the reasoning process, forming a traceable and step-wise verifiable reasoning chain.

\pincot{} encodes entities as lightweight XML tags. Two tag types are defined: \texttt{obj} for physical objects and \texttt{space} for task-relevant spatial regions. Both share a unified parameterized schema:

\begin{tcolorbox}[colback=gray!10!white, colframe=gray!50!black, arc=1pt, boxrule=0.5pt, left=4pt, right=4pt, top=4pt, bottom=4pt, halign=center]
\small\ttfamily
<obj name="NAME" id="ID" img\_idx="VIEW" point="[x, y]">\\
<space name="NAME" id="ID" img\_idx="VIEW" point="[x, y]">
\end{tcolorbox}


Here, \texttt{name} denotes a semantic label, \texttt{id} is an explicit identity token, \texttt{img\_idx} indicates the source view, and \texttt{point} represents a 2D coordinate normalized to the range 0--1000. Formally, each \reasoninganchor{} can be represented as a structured tuple $a = (n, i, v, p)$. This representation design tightly binds semantic meaning, identity information, view provenance, and spatial localization into a unified representation.

We adopt point coordinates over bounding boxes for three reasons. First, many embodied task targets are inherently about ``which location'' rather than ``which region'' (e.g., pointing, affordance prediction, placement positions), and points naturally align with such operational targets. Second, points are more compact: they incur lower information overhead when used as anchors within a reasoning chain. Third, the combination of point and ID is better suited as a reasoning variable, analogous to a pointer in a program that refers to a precise location while carrying identity, whereas a bounding box resembles an output of a detection module. We validate this design choice through ablation experiments comparing point and bounding box representations in Section~\ref{sec:ablation}.

Building on these structured tags, \pincot{} enforces an identity-aware reasoning mechanism. When an entity first appears during reasoning, it must be introduced through a complete XML tag that establishes both its spatial localization and identity. Subsequent reasoning steps reference the same entity directly through its ID, without regenerating a full tag.

This mechanism naturally extends to multi-view settings. The same entity observed across viewpoints shares a unified identity token, varying only in \texttt{img\_idx} and \texttt{point}. By enforcing a shared identity, cross-view consistency becomes an explicit constraint within the reasoning process, thereby reducing identity drift and enabling consistent reasoning about the same entity from different observation angles.


\subsection{Automated Data Construction}
\label{sec:data}

Training models to follow \pincot{} requires aligning visual grounding and identity with the reasoning process. However, existing multimodal datasets rarely provide such unified annotations, and directly converting raw data into \pincot{} format using large models tends to bypass explicit intermediate grounding steps, resulting in anchors that are not reliably grounded in visual evidence. We therefore build a fully automated three-stage pipeline organized around explicit structured intermediate representations, incorporating dedicated quality assurance throughout the process. Using this pipeline, we construct the \dataset{} reasoning dataset.

To identify task-relevant entities, we first use \teacher{}~\cite{bai2025qwen3} to analyze the current question and extract semantic descriptions of candidate entities. Since embodied task types vary significantly, a single prompting strategy cannot adequately cover all cases. We therefore partition the data into several task categories (e.g., spatial relation reasoning, pointing, affordance prediction) and design task-specific prompts for semantic parsing. This targeted strategy produces stable semantic specifications that accurately capture target entities.

Given the parsed semantic metadata, we employ a Florence-2~\cite{xiao2024florence} + SAM~2.1~\cite{ravi2024sam} pipeline to obtain precise point coordinates and bounding boxes for the relevant entities. This stage retains the predicted bounding boxes, refined segmentation masks, and derived point anchors as structured grounding evidence for subsequent use. However, this pipeline is not equally reliable across all target types: for small symbolic targets such as ``X'' marks in images, Florence-2 + SAM~2.1 often fails to localize accurately. To address this, we introduce a reverse prediction verification step, where Florence is asked to identify what the predicted point corresponds to. Only predictions whose reverse interpretation is consistent with the original target description are retained, substantially improving the quality and reliability of the grounding annotations.

We then feed the structured grounding evidence as ground-truth information into \teacher{} to generate the corresponding \pincot{} reasoning chains. To improve generation quality, we impose task-specific constraints for different task categories, reducing arbitrary or unsupported reasoning during generation. After obtaining \pincot{} outputs, we further apply rule-based filtering to remove low-quality reasoning chains and inconsistent results, such as incorrect ID references or mismatched anchor coordinates, ensuring the overall quality of the constructed data.


Through this three-stage pipeline, multimodal datasets are progressively transformed into structured reasoning data, in which visual evidence, entity identity, provenance, and answer supervision remain explicitly aligned throughout the construction process. The entire pipeline executes fully automatically without manual annotation and scales to large volumes of data, yielding the \dataset{} reasoning dataset.
Further details regarding the pipeline can be found in Appendix A.

\subsection{Progressive Training Pipeline}
\label{sec:training}

Building on the framework and data, we start from \student{}~\cite{bai2025qwen3} and progressively inject the capabilities through three-stage post-training: Stage~1 performs embodied domain adaptation via SFT, Stage~2 learns \pincot{} structured reasoning via CoT-SFT, and Stage~3 achieves process-supervised alignment via RFT.

% \textbf{Training Data}

We train \method{} on a diverse corpus to improve spatial understanding, multi-view reasoning, pointing, and long-horizon embodied reasoning. Different data subsets are assigned to different training stages according to their supervision signals and targeted capabilities. For Stage~2, we additionally apply the data construction pipeline described in Section~\ref{sec:data} to generate structured \pincot{} samples for learning \reasoninganchor{} introduction and the identity-aware reasoning mechanism.

\textbf{Geometric and general spatial reasoning data.}
This subset is primarily derived from \textbf{Euclid}~\cite{lian2025euclid} and \textbf{Video-R1}~\cite{feng2025video}. Euclid provides structured problems involving spatial relations and geometric properties, helping the model build precise spatial reasoning capabilities. Video-R1 provides general visual understanding samples from dynamic and diverse scenes, preserving the model's broad perceptual abilities during training.

\textbf{Embodied spatial reasoning and pointing data.}
This subset is primarily derived from \textbf{EmbSpatial}~\cite{du2024embspatial}, \textbf{EO-Data}~\cite{qu2025embodiedonevision}, \textbf{RoboVQA}~\cite{sermanet2024robovqa}, \textbf{EgoPlan}~\cite{chen2026egoplan}, and \textbf{Embodied-Point}~\cite{yuan2025embodied}. EmbSpatial and EO-Data focus primarily on embodied spatial perception, driving the model to develop robust environment-level reasoning capabilities. RoboVQA and EgoPlan textitasize task-oriented and egocentric embodied scenarios, introducing action-related reasoning and sequential decision-making processes. Furthermore, Embodied-Point covers diverse multi-task pointing scenarios, helping the model learn to generate precise point coordinates in embodied environments.

\textbf{Multi-view understanding data.}
This subset is primarily derived from \textbf{CrossPoint}~\cite{wang2025towards} and \textbf{SAT}~\cite{ray2024sat}, and augmented with additional multi-view data constructed from \textbf{InternData-M1}~\cite{contributors2025internroboticsrepo}. CrossPoint and SAT provide observations of the same scene under diverse camera viewpoints, enabling the model to learn consistent object representations and spatial relationships across views. InternData-M1 provides a diverse array of scenes, serving as a crucial foundation for multi-view reasoning in embodied tasks.

Detailed statistics of the training corpus, including the size of each data subset and the mixture ratios used across progressive training stages, are provided in Appendix B.


% \textbf{Stage 1 \& 2: From Embodied Adaptation to Structured Reasoning}

The first stage focuses on embodied domain adaptation. We fine-tune the model on embodied data covering object understanding, egocentric activity recognition, pointing and planning, enabling it to build foundational understanding of objects, affordances, spatial relations, and action events. A small amount of general-domain data is mixed in to mitigate catastrophic forgetting. The second stage injects \pincot{} structured reasoning ability. We leverage the pipeline from Section~\ref{sec:data} to generate structured, multi-step \pincot{} reasoning traces for supervised learning. In this stage, the model learns two key capabilities: introducing entities through complete XML tags to establish their \reasoninganchor{}s, and maintaining consistent identity references across both multi-step reasoning chains and multiple viewpoints.

% \textbf{Stage 3: RFT for Process-Supervised Alignment}

The third stage focuses on process-supervised alignment. After the first two stages, the model can generate structured reasoning chains, but may still prefer fluent yet poorly anchored outputs during inference. To counteract this tendency, we apply GRPO~\cite{shao2024deepseekmath} with a composite reward function that simultaneously supervises both the reasoning process and the final answer.

For a generated response $y$, let $\hat{a}$ denote the parsed final answer, $\mathcal{M}(y)$ the set of entity mentions appearing in the \texttt{<think>} block, and $\mathcal{M}_{\text{valid}}(y) \subseteq \mathcal{M}(y)$ the subset whose first occurrence is introduced by a valid format and whose subsequent mentions strictly maintain cross-step identity consistency. We further denote by $\mathcal{P}_{\text{xml}}(y)$ the set of anchor points extracted from the reasoning trace. For certain specific tasks, each predicted point $p_j$ is paired with a target grounding region $b_j^\star$.


We design a composite reward that evaluates four complementary dimensions of output quality:
\begin{equation}
R = \lambda_f R_{\text{format}} + \lambda_c R_{\text{consistency}} + \lambda_p R_{\text{pin}} + \lambda_a R_{\text{accuracy}},
\end{equation}
where $\lambda_\cdot$ are task-specific weights. When a reward term is not applicable to a particular task, its weight is set to zero.

\textbf{Format reward} $R_{\text{format}}$ evaluates whether the output structure is well-formed. The reasoning process must be enclosed within \texttt{<think>...</think>} and the answer within the format of \texttt{<answer>}...\texttt{</answer>}. The \texttt{<think>} block must also contain valid \reasoninganchor{} tags. The highest reward is assigned when both formatting and \reasoninganchor{} constraints are satisfied, a lower reward when only the outer format is correct, and zero otherwise.

\textbf{Consistency reward} $R_{\text{consistency}}$ evaluates the coherence of entity references throughout the reasoning process, measuring the proportion of entity mentions that follow the identity-aware reasoning mechanism:
\begin{equation}
R_{\text{consistency}} =
\frac{|\mathcal{M}_{\text{valid}}(y)|}{\max(|\mathcal{M}(y)|, 1)}.
\end{equation}
This reward encourages the model to maintain stable entity references across reasoning chains and multiple views, reducing identity drift and reference ambiguity.

\textbf{Pin reward} $R_{\text{pin}}$ evaluates the localization accuracy of \reasoninganchor{}s in the reasoning process. This term is applied only to datasets with explicit target region supervision, avoiding over-constraining the model's reasoning on other tasks:
\begin{equation}
R_{\text{pin}} =
\frac{\left| \left\{ p_j \in \mathcal{P}_{\text{xml}}(y) \mid p_j \in b_j^\star \right\} \right|}{\max(|\mathcal{P}_{\text{xml}}(y)|, 1)}.
\end{equation}
By directly supervising the localization accuracy of intermediate anchors, the pin reward ensures that \reasoninganchor{}s during reasoning are genuinely ``pinned'' to the correct locations.

\textbf{Accuracy reward} $R_{\text{accuracy}}$ evaluates the correctness of the final answer. Since answer formats vary across tasks, this reward is instantiated in a task-dependent manner: for multiple-choice tasks, it is a binary indicator of exact match; for pointing tasks, it measures the proportion of predicted points falling within the target bounding boxes; for open-ended tasks, it uses normalized sentence-level BLEU~\cite{papineni2002bleu} as a soft text-matching reward.


Overall, the reward design introduces process supervision over \textit{how the model reasons}. $R_{\text{format}}$ ensures well-formed outputs, $R_{\text{consistency}}$ enforces stable identity-aware reasoning mechanism, $R_{\text{pin}}$ directly supervises \reasoninganchor{} localization quality, and $R_{\text{accuracy}}$ ensures final-answer correctness. Together, these four terms enforce reasoning quality from both the process and the final answer, ultimately driving the model to generate high-quality \pincot{} reasoning chains. Further details regarding the training configurations can be found in Appendix C.   

==> ER_RoboPIN__Grounded_Embodied_Reasoning_via_Pinned_Chain_of_Thought/sections/relative_work.tex <==
% \section{Related Work}


% \subsection{Spatial Understanding and Reasoning}

% Spatial understanding and reasoning require vision-language models (VLMs) to infer object locations, spatial relations, and scene geometry from visual observations. This capability is critical for embodied AI applications such as navigation, interaction, and robotic manipulation. Recent studies have explored improving spatial reasoning in VLMs by introducing explicit spatial primitives, coordinate representations, or structured spatial relations. For example, SpatialVLM~\cite{chen2024spatialvlm} incorporates spatial coordinate systems to enhance geometric reasoning, while SpatialRGPT~\cite{cheng2024spatialrgpt} and SpatialBot~\cite{cai2025spatialbot} strengthen spatial reasoning through more precise modeling of object relations and scene structures. Beyond these representative works, TopViewRS~\cite{li2024topviewrs} studies top-view spatial reasoning, Reasoning Paths with Reference Objects~\cite{liao2024reasoning} demonstrates that explicitly introducing reference objects can elicit stronger quantitative spatial reasoning, and Visual Spatial Reasoning~\cite{liu2023visual} provides a broader analysis of spatial reasoning behavior in multimodal settings. In robotic manipulation, RoboPoint~\cite{yuan2024robopoint} predicts spatial affordance points for downstream control, FSD~\cite{yuan2025seeing} bridges reasoning and decision through affordance points and visual traces, and SpatialVLA~\cite{qu2025spatialvla} explores explicit spatial representations for vision-language-action models.

% \subsection{Visual Chain-of-Thought Reasoning}

% Chain-of-thought (CoT) prompting~\cite{wei2022chain} has substantially improved the reasoning ability of large language models by encouraging step-by-step intermediate reasoning. Subsequent works~\cite{zhang2022automatic,yao2023tree} extend this paradigm with various reasoning strategies and planning mechanisms. In multimodal reasoning, compositional CoT~\cite{mitra2024compositional} and DDCoT~\cite{zheng2023ddcot} further study how to structure intermediate reasoning paths and assign visual grounding responsibilities across steps.

% In the multimodal domain, several studies incorporate visual information into intermediate reasoning processes to improve interpretability and reasoning performance. For instance, Shikra~\cite{chen2023shikra} integrates region-based visual grounding into the reasoning process, while VoCoT~\cite{li2025vocot} extends visually grounded reasoning chains for multimodal tasks. VisualCoT~\cite{shao2024visual} provides a benchmark and evaluation framework for studying chain-of-thought reasoning in multi-hop visual question answering. Other works such as EmbodiedCoT~\cite{zawalski2024robotic}, FSD~\cite{yuan2025seeing}, and Embodied-R1~\cite{yuan2025embodied} extend structured intermediate reasoning to embodied environments for action-oriented decision making and control.

% \subsection{Multi-view Reasoning}

% Multi-view reasoning investigates how models integrate observations from multiple viewpoints and determine whether different visual inputs correspond to the same underlying scene elements. This capability is important in embodied intelligence scenarios where agents must reason over partial observations collected from different camera views or time steps.

% Recent work has explored multi-view reasoning in vision-language models by improving cross-view feature aggregation, representation alignment, or scene-level understanding. For example, CrossPoint~\cite{wang2025towards} studies cross-view point correspondence in VLMs, while MVRoboBench~\cite{feng2025seeing} benchmarks spatial reasoning in robotic scenes across different viewpoints. These approaches enable models to combine information from multiple perspectives and resolve viewpoint changes during reasoning. However, many existing systems still rely on implicit textual descriptions or latent representations to associate objects across views. Without explicit mechanisms for entity correspondence, verifying whether models consistently refer to the same physical object across observations can remain difficult, particularly in long-horizon reasoning scenarios.

\section{Related Work}


% \subsection{Spatial Understanding in Embodied Environments}

% Spatial understanding is crucial for embodied agents to bridge the "seeing-to-doing" gap~\cite{yuan2025embodied}. To achieve this, recent studies have significantly improved spatial reasoning by introducing explicit spatial primitives and coordinate representations. For example, SpatialVLM~\cite{chen2024spatialvlm} incorporates spatial coordinate systems to enhance geometric reasoning, while SpatialRGPT~\cite{cheng2024spatialrgpt} strengthens reasoning through precise modeling of scene structures. In the context of robotic manipulation, extracting actionable spatial representations is also critical; works like RoboPoint~\cite{yuan2024robopoint}, FSD~\cite{yuan2025seeing}, and SpatialVLA~\cite{qu2025spatialvla} predict spatial affordance points and visual traces to guide downstream control. 

% These advances provide a strong foundation for spatially grounded reasoning. 
% However, they are primarily designed for static or single-step settings, where spatial references are used locally within each prediction. In more realistic embodied scenarios, especially under multi-view observations, the difficulty increases as grounded references must remain stable across viewpoint changes and evolving observations. This requires not only accurate spatial localization, but also consistent identity tracking throughout the reasoning process. Building on this line of work, \method{} improves reasoning consistency in embodied settings through the proposed \pincot{} mechanism and process-supervised post-training, enabling persistent and identity-aware grounding across reasoning steps.

% \subsection{Embodied Spatial and Multi-View Reasoning}

% Spatial understanding is crucial for embodied agents to bridge the "seeing-to-doing" gap~\cite{yuan2025embodied}. To achieve this, recent studies have significantly improved spatial reasoning by  incorporating explicit spatial coordinates geometric reasoning  and scene structure modeling~\cite{chen2024spatialvlm,cheng2024spatialrgpt}. and predicting actionable points and visual traces for robotic manipulation\cite{yuan2024robopoint,yuan2025seeing,qu2025spatialvla}. However, these approaches primarily focus on static or single-view observations. In contrast, embodied environments are typically equipped with multiple viewpoints, necessitating that models integrate information across perspectives for comprehensive spatial understanding.

% Scaling to multi-view configurations, however, exposes critical vulnerabilities in spatial correspondence, as evidenced by recent benchmarks\cite{feng2025seeing,ray2024sat,wang2025towards}. A key challenge is that current grounded reasoning methods typically localize entities in a one-shot manner~\cite{chen2023shikra,you2023ferret,li2025vocot}, but lack a persistent mechanism for associating the same physical entity across diverse viewpoints. As a result, reasoning can become decoupled from visual evidence when viewpoint
% changes occur. To address this, our work introduces identity consistency to constrain the relationships between multi-view observations, effectively mitigating the decoupling of reasoning from visual evidence.

\subsection{Embodied Spatial Reasoning}

Spatial understanding is essential for embodied agents to bridge the ``seeing-to-doing'' gap.~\cite{yuan2025embodied}. To act reliably in physical environments, a model must not only recognize objects, but also infer their locations, spatial relations,
and task-relevant regions. Recent vision-language models have substantially improved this capability by incorporating explicit spatial coordinates, geometric reasoning, and scene-structure modeling into multimodal
representations~\cite{chen2024spatialvlm,cheng2024spatialrgpt}. In robotic manipulation settings, another important line of work predicts actionable points and visual traces that can directly support downstream control, such as grasping, placing, or interaction
planning~\cite{yuan2024robopoint,yuan2025seeing,qu2025spatialvla}. Together, these efforts have significantly strengthened embodied models in tasks such as spatial referring, target localization, and manipulation-oriented grounding.

\subsection{Embodied Multi-View Reasoning}

To alleviate the occlusion and partial visibility issues inherent to single-view observations, multi-view configurations have become a standard paradigm in embodied perception and manipulation~\cite{jangir2022look,jang2023murm}. Existing embodied foundation models~\cite{kim2024openvla,team2024octo} typically integrate these multi-view inputs through feature concatenation, cross-view attention mechanisms, or unified encoders to enhance overall scene coverage and spatial awareness.
However, the core challenge of multi-view reasoning extends beyond mere information fusion; it inherently demands robust \textit{cross-view correspondence}. A model must reliably determine whether distinct regions or entities across disparate views correspond to the same physical target. Recent multi-view benchmarks~\cite{feng2025seeing,wang2025towards,ray2024sat} reveal that current vision-language models remain highly fragile in this capability. When faced with drastic shifts in perspective, scale, and visibility, they often fail to consistently associate the same entity. The fundamental root cause is that most existing grounded reasoning methods predominantly produce localized, one-off spatial references, lacking a persistent identity-binding mechanism. Our work explicitly addresses this bottleneck by enforcing ID consistency constraints across multi-view observations, ensuring reliable and persistent entity alignment.


% Without an explicit mechanism to bridge these visual discrepancies, the reasoning process becomes decoupled from consistent visual evidence, ultimately hindering the agent’s capacity for reliable long-horizon interactions.

\subsection{Visually Grounded Chain-of-Thought}

Chain-of-Thought (CoT)~\cite{wei2022chain} significantly enhances the reasoning abilities of large language models. To extend this paradigm to multimodal domains, early works primarily focused on augmenting the intermediate reasoning process with visual evidence\cite{zhang2023multimodal,zhang2023multimodal,zheng2023ddcot}. While these methods successfully improve interpretability, their reasoning processes remain predominantly text-centric.

To better leverage visual information within reasoning, subsequent methods progressed by directly injecting spatial references into the reasoning chain\cite{chen2023shikra,you2023ferret,li2025vocot}. However, while these methods successfully make visual grounding explicit, they predominantly treat spatial references as localized, single-use annotations attached to individual reasoning steps. Consequently, entity tracking still relies on implicit natural language descriptions, leaving current models highly susceptible to cross-step reference drift. Our work addresses this limitation by introducing the \reasoninganchor{}. By representing grounded entities as persistent, identity-bound anchors, we make intermediate references trackable across steps.

% \subsection{Process Supervision for Embodied Reasoning}

% While process supervision~\cite{lightman2023let} has significantly improved LLM reliability by evaluating intermediate steps, extending it to embodied vision-language models (VLMs) remains challenging. Most embodied models still rely on outcome supervision, risking correct final actions derived from incorrect spatial grounding. The key bottleneck for process supervision in VLMs is that intermediate reasoning is predominantly implicit or expressed through unconstrained free-form text. This makes it exceedingly difficult to programmatically verify which entity the model refers to at each step, severely hindering the definition of dense process rewards.

% Our work addresses this limitation by exposing intermediate reasoning as explicit \reasoninganchor{}s. By representing entities with precise spatial coordinates and persistent identity binding, we enable the design of explicit reward functions for intermediate steps, thereby successfully achieving process supervision.

==> ER_RoboPIN__Grounded_Embodied_Reasoning_via_Pinned_Chain_of_Thought/sections/training.tex <==
\section{Training}
\label{sec:training}

In this section, we start from \student\ and progressively equip it with the required capabilities through a three-stage fine-tuning pipeline.

\subsection{Training Data}

We train \student\ on a diverse corpus to improve spatial understanding, multi-view reasoning, pointing, and long-horizon embodied reasoning. Different data sources are assigned to different training stages according to their supervision signals and targeted capabilities. For the Stage~2, we further apply our data construction pipeline to generate structured VIA-CoT samples for learning visual anchoring, identity tracking, and multi-step reasoning.

\textbf{Geometric and General Spatial Reasoning Data.}
We construct a dedicated subset to enhance the model’s geometric and spatial reasoning capabilities while maintaining its general visual understanding. This subset is primarily derived from \textbf{Euclid}~\cite{lian2025euclid} and \textbf{Video-R1}~\cite{video-r1}. (1) \textbf{Euclid} serves as the primary source for geometric reasoning. It provides structured problems involving spatial relations and geometric properties, which help the model develop a more precise understanding of object layouts and spatial constraints. (2) \textbf{Video-R1} focuses on general visual understanding in dynamic and diverse scenes. These samples are incorporated to preserve the model’s broader perception during training.

\textbf{Embodied Spatial Data.}
We construct a dedicated subset of embodied spatial data to inject knowledge of physical environments, spatial perception, and task-oriented interaction. This subset is primarily derived from \textbf{SAT}~\cite{ray2024sat}, \textbf{EmbSpatial}~\cite{du2024embspatial}, \textbf{EO-Data}~\cite{qu2025embodiedonevision}, \textbf{RoboVQA}~\cite{sermanet2024robovqa}, and \textbf{EgoPlan}~\cite{chen2026egoplan}. (1) \textbf{SAT}, \textbf{EmbSpatial}, and \textbf{EO-Data} mainly focus on spatial perception and environment-level reasoning. They provide diverse annotations of object-centric spatial relations, scene layouts, and region-level interactions, enabling the model to better understand how objects are arranged and related within complex environments. (2) \textbf{RoboVQA} and \textbf{EgoPlan} emphasize task-oriented and egocentric embodied scenarios. These datasets introduce action-related reasoning, agent-centric observations, and sequential decision-making processes, helping the model capture how agents perceive, plan, and interact with their surroundings.

\textbf{Multi-View Understanding Data.}
To enhance multi-view reasoning ability in embodied scenarios, we include a dedicated subset focusing on cross-view perception and spatial consistency. This subset is primarily derived from \textbf{CrossPoint}~\cite{wang2025towards} and augmented with additional multi-view data from \textbf{InternData-M1}~\cite{InternData}. (1) \textbf{CrossPoint} serves as the primary source for multi-view understanding. It provides observations of the same scene under diverse camera viewpoints, enabling the model to learn consistent object representations and spatial relationships across views. (2) \textbf{InternData-M1} is used to construct additional multi-view reasoning data tailored to embodied tasks. It broadens the diversity of scenes and interaction patterns, helping the model generalize multi-view reasoning to more complex and task-oriented settings. 



\subsection{Stage 1: SFT for Embodied Adaptation}
The first stage focuses on adapting the base model to embodied domains. We fine-tune the model on embodied supervision covering object-centric understanding, egocentric activities, pointing, planning, and question answering. These data expose the model to common physical scenes, interaction patterns, and action-relevant visual cues, helping it build fundamental grounding for objects, affordances, spatial relations, and motion events. To avoid degrading the model's original general-purpose capabilities during domain adaptation, we additionally mix a small amount of general-domain supervision in this stage, which helps preserve its broad visual-language competence and mitigates catastrophic forgetting. This stage serves as the foundation of the entire training pipeline, preparing the model for the subsequent learning of structured reasoning grounded in explicit visual anchoring and consistent ID tracking.

\subsection{Stage 2: LongSFT for Structured Long-Horizon Reasoning}
The second stage is designed to equip the model with the structured reasoning ability required by embodied and multi-view tasks. To this end, we leverage our efficient CoT construction pipeline to build long-form training traces for embodied-domain and multi-view reasoning, and use them to supervise reasoning under the proposed visual anchoring and ID-tracking paradigm. In this stage, the model learns to introduce entities through explicit visual anchors, maintain consistent ID references across extended reasoning chains, and reuse shared IDs across views when the same physical entity is observed multiple times. 

\subsection{Stage 3: RFT for Policy Alignment}
The third stage focuses on policy-level alignment. After the first two stages, the model is able to produce structured reasoning traces, but it may still prefer fluent yet weakly anchored outputs at inference time. To further strengthen its reasoning behavior, we apply GRPO~\cite{shao2024deepseekmath} on the subset of training data for which reliable verification signals can be defined. Specifically, the optimization rewards four complementary aspects of the response: format compliance, spatial accuracy of intermediate grounding during reasoning, consistency of subsequent ID references, and final answer correctness. In this way, the robustness and reliability of the model outputs are effectively improved.

\subsubsection{Reward Design}
To prevent the model from merely producing placeholder structured outputs rather than performing effective grounded reasoning, we design a task-dependent composite reward in the RFT stage that explicitly supervises visual anchoring and ID tracking:
\begin{equation}
R = \lambda_f R_{\text{format}} + \lambda_c R_{\text{consistency}} + \lambda_s R_{\text{spatial}} + \lambda_a R_{\text{accuracy}},
\end{equation}
where $\lambda_\cdot$ are task-specific weights. If a reward term is not applicable to a task, its weight is set to zero. The four reward terms are designed to evaluate complementary aspects of the output: structural validity, entity consistency, spatial grounding, and final-answer correctness.

For a generated response $y$, let $\hat{a}$ denote the parsed final answer, $\mathcal{M}(y)$ the set of entity mentions appearing in the \texttt{<think>} block, and $\mathcal{M}_{\text{valid}}(y) \subseteq \mathcal{M}(y)$ the subset whose first occurrence is introduced by a valid XML anchor and whose subsequent references reuse the corresponding ID consistently. We further denote by $\mathcal{P}_{\text{xml}}(y)$ the set of anchor points extracted from the reasoning trace and by $\mathcal{P}_{\text{ans}}(y)$ the set of points extracted from the final answer. For tasks with spatial supervision, each predicted point $p_j$ is paired with a target grounding region $b_j^\star$.


\textbf{Format reward.}
To encourage well-formed structured outputs, we define a format reward $R_{\text{format}}$ that evaluates whether the response follows the prescribed reasoning schema. Specifically, the reasoning process must be enclosed within \texttt{<think>...</think>} and the final answer must be wrapped in \texttt{<answer>...</answer>}. Moreover, the \texttt{<think>} block is required to contain visual anchors of the form \texttt{<obj/space name="" id="" img\_idx="" point="[]">}, which explicitly bind objects or spaces to grounded image coordinates. In practice, we assign the highest reward when both the global response format and the XML-anchor constraints are satisfied, a slightly lower reward when only the outer response format is correct, and zero reward otherwise. This reward encourages the model to produce parseable reasoning traces with explicit visual grounding, rather than superficial placeholder content.

\textbf{Consistency reward.}
To encourage stable reasoning over entities, we define a consistency reward $R_{\text{consistency}}$ that evaluates whether visual anchors and subsequent ID references remain coherent throughout the reasoning trajectory. Concretely, we measure the ratio of entity mentions that follow the prescribed XML introduction and ID reuse rules:
\begin{equation}
R_{\text{consistency}} =
\frac{|\mathcal{M}_{\text{valid}}(y)|}{\max(|\mathcal{M}(y)|, 1)}.
\end{equation}
This reward favors responses in which entities are introduced clearly and tracked consistently over long chains of reasoning and across multiple views, thereby reducing identity drift and reference ambiguity.

\textbf{Spatial reward.}
To encourage physically grounded reasoning, we define a spatial reward $R_{\text{spatial}}$. To avoid over-constraining the model's reasoning process, we apply this reward only to datasets with explicit object-level supervision signals, where the grounded target region can be unambiguously determined. This term evaluates whether the intermediate visual anchors produced in the reasoning process are consistent with the target grounded regions:
\begin{equation}
R_{\text{spatial}} =
\frac{\left| \left\{ p_j \in \mathcal{P}_{\text{xml}}(y) \mid p_j \in b_j^\star \right\} \right|}{\max(|\mathcal{P}_{\text{xml}}(y)|, 1)}.
\end{equation}
By rewarding accurate intermediate grounding on these supervised samples, the spatial reward directly supervises the quality of the \texttt{<think>} process rather than only the correctness of the final answer.

\textbf{Accuracy reward.}
To preserve task success, we define an accuracy reward $R_{\text{accuracy}}$ that measures the consistency between the predicted answer and the task target. Since the final-answer format differs across tasks, we instantiate this reward in a task-dependent way. For multiple-choice tasks, the reward is binary and indicates whether the predicted option exactly matches the ground-truth answer. For pointing tasks, the reward is defined as the ratio of predicted final-answer points that fall inside the corresponding target bounding boxes. For open-ended tasks, we use normalized sentence-level BLEU as a soft text-matching reward, which provides non-binary supervision even when the generated answer differs slightly in surface form from the reference. This reward provides a direct optimization signal for final-answer correctness and complements the other reward terms, which mainly regulate the quality of the reasoning process.

Overall, the reward design separates \emph{how the model reasons} from \emph{what the model answers}: $R_{\text{format}}$ encourages well-formed outputs, $R_{\text{consistency}}$ enforces stable ID tracking, $R_{\text{spatial}}$ supervises intermediate visual grounding, and $R_{\text{accuracy}}$ ensures final-answer correctness.


% \begin{figure}[t]
%   \centering
%   \IfFileExists{figure/reward_design.png}{
%     \includegraphics[width=\linewidth]{figure/reward_design.png}
%   }{
%     \fbox{\parbox{0.96\linewidth}{\vspace{0.25cm}\centering Placeholder: \texttt{reward\_design.png}\vspace{0.25cm}}}
%   }
%   \caption{Overview of the reward design}
%   \label{fig:reward}
% \end{figure}


==> Makefile <==
TEX = main

.PHONY: all clean

all: $(TEX).pdf

$(TEX).pdf: $(TEX).tex sample-base.bib sections/*.tex iffyuan.cls
	pdflatex -interaction=nonstopmode $(TEX).tex
	bibtex $(TEX)
	pdflatex -interaction=nonstopmode $(TEX).tex
	pdflatex -interaction=nonstopmode $(TEX).tex

clean:
	$(RM) $(TEX).aux $(TEX).bbl $(TEX).blg $(TEX).log $(TEX).out \
	      $(TEX).toc $(TEX).lof $(TEX).lot $(TEX).fls $(TEX).fdb_latexmk \
	      $(TEX).synctex.gz


==> sections/ablations.tex <==
\section{Ablation Study and Analysis}

In this section, we conduct ablation experiments in both embodied reasoning and multi-view reasoning settings to examine whether the performance gains of our model mainly arise from the proposed structured VIA-CoT design and the subsequent RFT optimization. To this end, we construct several model variants with different reasoning supervision formats and training strategies, and evaluate them on the corresponding benchmarks in each scenario. By comparing the resulting performance changes, we analyze the contribution of VIA-CoT and RFT to the final model performance.

\noindent\textbf{Experimental Setup.}
We compare eight configurations built around the Qwen3-VL-4B model family. The original Qwen3-VL-4B-Instruct serves as the base model for all supervised training variants and also provides the primary training baseline without any additional adaptation. We further include the off-the-shelf Qwen3-VL-4B-Thinking model as a reference baseline to compare against a native reasoning model.

Starting from each sampled ablation subset, we construct three supervision formats from the same underlying image--question--answer instances. The first is a \textbf{Direct} dataset that contains only the final answers and is used to train a standard QA model without intermediate reasoning. The second is a \textbf{CoT} dataset, where chain-of-thought traces are generated by Qwen3-VL-32B-Instruct. The third is a \textbf{VIA-CoT} dataset produced by our current pipeline, which provides structured reasoning traces with explicit visual anchors and identity tracking. For each supervision format, we evaluate both an SFT-only variant and a corresponding RFT-enhanced variant when applicable, yielding six trained variants in total. Across all ablation settings, except for differences in supervision format and the optional RFT stage, the remaining training-related settings are kept identical to ensure a controlled comparison.



\subsection{Embodied Reasoning Ablations}

We conduct the embodied reasoning ablation study on \textbf{EmbSpatial}, which is accompanied by corresponding data targeting embodied spatial reasoning capabilities.
For comparison, we extract a fixed evaluation subset consisting of 25K samples from EmbSpatial.

\begin{table}[htbp]
  \centering
  \small
  \setlength{\tabcolsep}{6pt}
  \caption{Embodied ablations on EmbSpatial.}
  \label{tab:embodied_ablation_main}
  \begin{tabular}{lc}
    \toprule
    Model & Accuracy $\uparrow$ \\
    \midrule
    Qwen3-VL-4B-Instruct & 77.1 \\
    Qwen3-VL-4B-Thinking & 78.9 \\
    \midrule
    Direct & 76.00 \\
    \hspace{0.8em}w/o RFT & 75.1 \\
    CoT & 79.23 \\
    \hspace{0.8em}w/o RFT & 79.1 \\
    \rowcolor{blue!10} VIA-CoT & \textbf{84.7} \\
    \hspace{0.8em}w/o RFT & 80.3 \\
    \bottomrule
  \end{tabular}
\end{table}


\subsection{Multi-view Reasoning Ablations}

We further evaluate the impact of structured reasoning in the multi-view setting on the \textbf{SAT} benchmark, where we focus on the \textbf{ego\_movement} and \textbf{obj\_movement} subtasks.
For comparison, we construct fixed evaluation subsets from these two SAT subtasks and evaluate all supervision variants under the same protocol.

\begin{table}[htbp]
  \centering
  \small
  \setlength{\tabcolsep}{6pt}
  \caption{Multi-view ablations on the SAT \textit{ego\_movement} and \textit{obj\_movement} subtasks.}
  \label{tab:multiview_ablation}
  \begin{tabular}{lcc}
    \toprule
    Model & \shortstack{ego\_movement\\Accuracy $\uparrow$} & \shortstack{obj\_movement\\Accuracy $\uparrow$} \\
    \midrule
    Qwen3-VL-4B-Instruct & 79.3 & 39.1 \\
    Qwen3-VL-4B-Thinking & 82.6 & 60.9 \\
    \midrule
    Direct & 73.9 & 60.8 \\
    \hspace{0.8em}w/o RFT & 39.1 & 39.1 \\
    CoT & \textbf{100} & 82.6 \\
    \hspace{0.8em}w/o RFT & 91.3 & 73.9 \\
    \rowcolor{blue!10} VIA-CoT & \textbf{100} & \textbf{87.0} \\
    \hspace{0.8em}w/o RFT & 87.0 & 78.3 \\
    \bottomrule
  \end{tabular}
\end{table}


\subsection{Reward Function Ablations}

To further isolate the contribution of individual reward terms introduced in Section~\ref{sec:training}, we conduct a reward-function ablation study in the same embodied setting as above. Concretely, we reuse the same EmbSpatial training data and the same fixed 25K-sample EmbSpatial evaluation subset used in the embodied reasoning ablations. All training and evaluation settings are kept identical to the full VIA-CoT + RFT model, except that we remove one reward term at a time during Stage 3 RFT.

In particular, we examine two reward components that are directly related to the proposed grounded reasoning behavior: the spatial reward $R_{\text{spatial}}$, which supervises intermediate visual grounding, and the ID-tracking reward $R_{\text{consistency}}$, which encourages consistent entity references throughout the reasoning trajectory. The format reward and accuracy reward are kept unchanged in these ablations.

\begin{table}[htbp]
  \centering
  \small
  \setlength{\tabcolsep}{6pt}
  \caption{Reward-function ablations on EmbSpatial.}
  \label{tab:reward_ablation_embodied}
  \begin{tabular}{lc}
    \toprule
    Model & Accuracy $\uparrow$ \\
    \midrule
     VIA-CoT & \textit{80.3} \\
    \rowcolor{blue!10} VIA-CoT + RFT & \textit{84.7} \\
    \hspace{0.8em}w/o Spatial Reward & 81.2 \\
    \bottomrule
  \end{tabular}
\end{table}

This ablation is designed to distinguish whether the gains from RFT mainly come from better intermediate spatial grounding or from more stable ID tracking. After the results are filled in, the relative performance drop of each variant can be used to quantify the importance of the corresponding reward component under the embodied evaluation setting.



\subsection{Analysis.}
The results reveal a clear trend as the reasoning format becomes more structured. 
Direct supervision provides limited support for multi-step reasoning in multi-view settings. 
Introducing chain-of-thought reasoning improves performance by exposing intermediate reasoning steps. 
Structured VIA-CoT further enhances performance by explicitly grounding reasoning steps to visual anchors and maintaining consistent object identities across views. 
Finally, reinforcement fine-tuning provides additional gains by aligning reasoning trajectories with task-level objectives.

==> sections/training.tex <==
\section{Training}
\label{sec:training}

In this section, we start from \student\ and progressively equip it with the required capabilities through a three-stage fine-tuning pipeline.

\subsection{Training Data}

We train \student\ on a diverse corpus to improve spatial understanding, multi-view reasoning, pointing, and long-horizon embodied reasoning. Different data sources are assigned to different training stages according to their supervision signals and targeted capabilities. For the Stage~2, we further apply our data construction pipeline to generate structured VIA-CoT samples for learning visual anchoring, identity tracking, and multi-step reasoning.

\textbf{Geometric and General Spatial Reasoning Data.}
We construct a dedicated subset to enhance the model’s geometric and spatial reasoning capabilities while maintaining its general visual understanding. This subset is primarily derived from \textbf{Euclid}~\cite{lian2025euclid} and \textbf{Video-R1}~\cite{video-r1}. (1) \textbf{Euclid} serves as the primary source for geometric reasoning. It provides structured problems involving spatial relations and geometric properties, which help the model develop a more precise understanding of object layouts and spatial constraints. (2) \textbf{Video-R1} focuses on general visual understanding in dynamic and diverse scenes. These samples are incorporated to preserve the model’s broader perception during training.

\textbf{Embodied Spatial Data.}
We construct a dedicated subset of embodied spatial data to inject knowledge of physical environments, spatial perception, and task-oriented interaction. This subset is primarily derived from \textbf{SAT}~\cite{ray2024sat}, \textbf{EmbSpatial}~\cite{du2024embspatial}, \textbf{EO-Data}~\cite{qu2025embodiedonevision}, \textbf{RoboVQA}~\cite{sermanet2024robovqa}, and \textbf{EgoPlan}~\cite{chen2026egoplan}. (1) \textbf{SAT}, \textbf{EmbSpatial}, and \textbf{EO-Data} mainly focus on spatial perception and environment-level reasoning. They provide diverse annotations of object-centric spatial relations, scene layouts, and region-level interactions, enabling the model to better understand how objects are arranged and related within complex environments. (2) \textbf{RoboVQA} and \textbf{EgoPlan} emphasize task-oriented and egocentric embodied scenarios. These datasets introduce action-related reasoning, agent-centric observations, and sequential decision-making processes, helping the model capture how agents perceive, plan, and interact with their surroundings.

\textbf{Multi-View Understanding Data.}
To enhance multi-view reasoning ability in embodied scenarios, we include a dedicated subset focusing on cross-view perception and spatial consistency. This subset is primarily derived from \textbf{CrossPoint}~\cite{wang2025towards} and augmented with additional multi-view data from \textbf{InternData-M1}~\cite{InternData}. (1) \textbf{CrossPoint} serves as the primary source for multi-view understanding. It provides observations of the same scene under diverse camera viewpoints, enabling the model to learn consistent object representations and spatial relationships across views. (2) \textbf{InternData-M1} is used to construct additional multi-view reasoning data tailored to embodied tasks. It broadens the diversity of scenes and interaction patterns, helping the model generalize multi-view reasoning to more complex and task-oriented settings. 



\subsection{Stage 1: SFT for Embodied Adaptation}
The first stage focuses on adapting the base model to embodied domains. We fine-tune the model on embodied supervision covering object-centric understanding, egocentric activities, pointing, planning, and question answering. These data expose the model to common physical scenes, interaction patterns, and action-relevant visual cues, helping it build fundamental grounding for objects, affordances, spatial relations, and motion events. To avoid degrading the model's original general-purpose capabilities during domain adaptation, we additionally mix a small amount of general-domain supervision in this stage, which helps preserve its broad visual-language competence and mitigates catastrophic forgetting. This stage serves as the foundation of the entire training pipeline, preparing the model for the subsequent learning of structured reasoning grounded in explicit visual anchoring and consistent ID tracking.

\subsection{Stage 2: LongSFT for Structured Long-Horizon Reasoning}
The second stage is designed to equip the model with the structured reasoning ability required by embodied and multi-view tasks. To this end, we leverage our efficient CoT construction pipeline to build long-form training traces for embodied-domain and multi-view reasoning, and use them to supervise reasoning under the proposed visual anchoring and ID-tracking paradigm. In this stage, the model learns to introduce entities through explicit visual anchors, maintain consistent ID references across extended reasoning chains, and reuse shared IDs across views when the same physical entity is observed multiple times. 

\subsection{Stage 3: RFT for Policy Alignment}
The third stage focuses on policy-level alignment. After the first two stages, the model is able to produce structured reasoning traces, but it may still prefer fluent yet weakly anchored outputs at inference time. To further strengthen its reasoning behavior, we apply GRPO~\cite{shao2024deepseekmath} on the subset of training data for which reliable verification signals can be defined. Specifically, the optimization rewards four complementary aspects of the response: format compliance, spatial accuracy of intermediate grounding during reasoning, consistency of subsequent ID references, and final answer correctness. In this way, the robustness and reliability of the model outputs are effectively improved.

\subsubsection{Reward Design}
To prevent the model from merely producing placeholder structured outputs rather than performing effective grounded reasoning, we design a task-dependent composite reward in the RFT stage that explicitly supervises visual anchoring and ID tracking:
\begin{equation}
R = \lambda_f R_{\text{format}} + \lambda_c R_{\text{consistency}} + \lambda_s R_{\text{spatial}} + \lambda_a R_{\text{accuracy}},
\end{equation}
where $\lambda_\cdot$ are task-specific weights. If a reward term is not applicable to a task, its weight is set to zero. The four reward terms are designed to evaluate complementary aspects of the output: structural validity, entity consistency, spatial grounding, and final-answer correctness.

For a generated response $y$, let $\hat{a}$ denote the parsed final answer, $\mathcal{M}(y)$ the set of entity mentions appearing in the \texttt{<think>} block, and $\mathcal{M}_{\text{valid}}(y) \subseteq \mathcal{M}(y)$ the subset whose first occurrence is introduced by a valid XML anchor and whose subsequent references reuse the corresponding ID consistently. We further denote by $\mathcal{P}_{\text{xml}}(y)$ the set of anchor points extracted from the reasoning trace and by $\mathcal{P}_{\text{ans}}(y)$ the set of points extracted from the final answer. For tasks with spatial supervision, each predicted point $p_j$ is paired with a target grounding region $b_j^\star$.


\textbf{Format reward.}
To encourage well-formed structured outputs, we define a format reward $R_{\text{format}}$ that evaluates whether the response follows the prescribed reasoning schema. Specifically, the reasoning process must be enclosed within \texttt{<think>...</think>} and the final answer must be wrapped in \texttt{<answer>...</answer>}. Moreover, the \texttt{<think>} block is required to contain visual anchors of the form \texttt{<obj/space name="" id="" img\_idx="" point="[]">}, which explicitly bind objects or spaces to grounded image coordinates. In practice, we assign the highest reward when both the global response format and the XML-anchor constraints are satisfied, a slightly lower reward when only the outer response format is correct, and zero reward otherwise. This reward encourages the model to produce parseable reasoning traces with explicit visual grounding, rather than superficial placeholder content.

\textbf{Consistency reward.}
To encourage stable reasoning over entities, we define a consistency reward $R_{\text{consistency}}$ that evaluates whether visual anchors and subsequent ID references remain coherent throughout the reasoning trajectory. Concretely, we measure the ratio of entity mentions that follow the prescribed XML introduction and ID reuse rules:
\begin{equation}
R_{\text{consistency}} =
\frac{|\mathcal{M}_{\text{valid}}(y)|}{\max(|\mathcal{M}(y)|, 1)}.
\end{equation}
This reward favors responses in which entities are introduced clearly and tracked consistently over long chains of reasoning and across multiple views, thereby reducing identity drift and reference ambiguity.

\textbf{Spatial reward.}
To encourage physically grounded reasoning, we define a spatial reward $R_{\text{spatial}}$. To avoid over-constraining the model's reasoning process, we apply this reward only to datasets with explicit object-level supervision signals, where the grounded target region can be unambiguously determined. This term evaluates whether the intermediate visual anchors produced in the reasoning process are consistent with the target grounded regions:
\begin{equation}
R_{\text{spatial}} =
\frac{\left| \left\{ p_j \in \mathcal{P}_{\text{xml}}(y) \mid p_j \in b_j^\star \right\} \right|}{\max(|\mathcal{P}_{\text{xml}}(y)|, 1)}.
\end{equation}
By rewarding accurate intermediate grounding on these supervised samples, the spatial reward directly supervises the quality of the \texttt{<think>} process rather than only the correctness of the final answer.

\textbf{Accuracy reward.}
To preserve task success, we define an accuracy reward $R_{\text{accuracy}}$ that measures the consistency between the predicted answer and the task target. Since the final-answer format differs across tasks, we instantiate this reward in a task-dependent way. For multiple-choice tasks, the reward is binary and indicates whether the predicted option exactly matches the ground-truth answer. For pointing tasks, the reward is defined as the ratio of predicted final-answer points that fall inside the corresponding target bounding boxes. For open-ended tasks, we use normalized sentence-level BLEU as a soft text-matching reward, which provides non-binary supervision even when the generated answer differs slightly in surface form from the reference. This reward provides a direct optimization signal for final-answer correctness and complements the other reward terms, which mainly regulate the quality of the reasoning process.

Overall, the reward design separates \emph{how the model reasons} from \emph{what the model answers}: $R_{\text{format}}$ encourages well-formed outputs, $R_{\text{consistency}}$ enforces stable ID tracking, $R_{\text{spatial}}$ supervises intermediate visual grounding, and $R_{\text{accuracy}}$ ensures final-answer correctness.


% \begin{figure}[t]
%   \centering
%   \IfFileExists{figure/reward_design.png}{
%     \includegraphics[width=\linewidth]{figure/reward_design.png}
%   }{
%     \fbox{\parbox{0.96\linewidth}{\vspace{0.25cm}\centering Placeholder: \texttt{reward\_design.png}\vspace{0.25cm}}}
%   }
%   \caption{Overview of the reward design}
%   \label{fig:reward}
% \end{figure}

